Microwave dielectric properties of LiNbO$_{\mathbf{3}}$ and AlN at millikelvin temperatures and single-photon power

Efficient bidirectional microwave-optical photon conversion is a key capability for scaling superconducting quantum processors into distributed networks. However, achieving the necessary conversion efficiency requires filling a critical knowledge gap in understanding the loss mechanisms of electro-optic materials. Here, we characterize the microwave properties of single-crystal bulk LiNbO3 and AlN over a broad range of powers, down to single-photon levels, and spanning from millikelvin temperatures to above 1 K. We demonstrate that both materials exhibit two-level systems (TLS) behavior, while piezoelectric-related losses are excluded. We show that TLS-induced dissipation is predominantly localized on the surface rather than being an intrinsic bulk property, a result further corroborated by room-temperature 3D XPS and time-of-flight SIMS analyses. These findings provide useful insights to engineer hybrid architectures that integrate bulk electro-optic crystals within superconducting cavities, proving that microwave quality factors compatible with high-efficiency microwave-optical transduction are within reach.

==> Tables/Loss_tangent_from_power_sweeps.tex <==
\begin{sidewaystable}[htbp!]
\begin{threeparttable}
    \centering
    \caption{TLS loss tangent results from single-photon internal quality factor measurements at base temperature ($T_{\mathrm{MXC}} = 8 $ mK).}
    \begin{tabular*}{0.84\textwidth}{@{}lcccccc@{}}
    \toprule
    Sample & $\nu_{0,\parallel}$ [GHz] & $p_{\parallel}$ & $\tan\delta_{\parallel,\mathrm{TLS,0}}$ & $\nu_{0,\perp}$ [GHz] & $p_{\perp}$ & $\tan\delta_{\perp,\mathrm{TLS,0}}$ \\
    \midrule
        AlN & 9.56 $\pm$ 0.01 & 0.49 $\pm$ 0.01 & (5.7 $\pm$ 0.2)$\times10^{-6}$ & 15.51 $\pm$ 0.01 & 0.933 $\pm$ 0.008 & (1.5 $\pm$ 0.1)$\times 10^{-6}$ \\
        LiNbO$_{3}$ & 7.676 $\pm$ 0.001 & 0.45 $\pm$ 0.02 & (2.9 $\pm$ 0.1)$\times10^{-6}$ & 7.022 $\pm$ 0.001 & 0.941 $\pm$ 0.002 & (2.92 $\pm$ 0.02)$\times 10^{-6}$\\
    \bottomrule
    \end{tabular*}
    \label{tab:LossTanSinglePhResults}
\end{threeparttable}
\end{sidewaystable}


==> Tables/Power_sweep_regression_results_TE011_comparison.tex <==
\begin{center}
\begin{threeparttable}[htbp!]
    \centering
    \caption{Piecewise fit results of the TE$_{011}$ mode internal quality factor towards power data series of the two materials for different DR runs.}
    \begin{tabular*}{0.88\textwidth}{@{}lcccc@{}}
    \toprule
    Sample & $Q_{\mathrm{TLS,0}}$ & $P_{c}$ [dBm] & $\beta$ & $Q_{\mathrm{other}}$ & $Q_{0}\left(\bar{n}_{ph}\rightarrow0\right)$ \\
    \midrule
        AlN\tnote{1} & (7.2 $\pm$ 0.6)$\times 10^{5}$ & -75 $\pm$ 1 & 1.4 $\pm$ 0.5 & (7.8 $\pm$ 0.3)$\times 10^{4}$ & (7.0 $\pm$ 0.4)$\times 10^{4}$\\
        LiNbO$_{3}$\tnote{2} & (3.64 $\pm$ 0.03)$\times 10^{5}$ & -84.9 $\pm$ 0.2 & 1.05 $\pm$ 0.03 & (5.38 $\pm$ 0.04)$\times 10^{4}$ & (4.68 $\pm$ 0.04)$\times 10^{4}$
    \bottomrule
    \end{tabular*}
    \begin{tablenotes}
        \item [1]{Resonance frequency $\nu_{0}=$ 15.508453(4) GHz}
        \item [2]{Resonance frequency $\nu_{0}=$ 7.020667(1) GHz}
    \end{tablenotes}
    
    \label{tab:PwrSweepRegrResultsTE011}
\end{threeparttable}
\end{center}

==> Tables/Power_sweep_regression_results_TM010_comparison.tex <==
\begin{sidewaystable}[htbp!]
\begin{threeparttable}
    \centering
    \caption{Piecewise fit results of the TM$_{010}$ mode internal quality factor towards power data series of the two materials for different DR runs.}
    \begin{tabular*}{0.9\textwidth}{@{}ll@{}cccccc@{}}
    \toprule
    Sample & Run n. & $Q_{\mathrm{TLS,0}}$ & $P_{c}$ [dBm] & $\beta$ & $Q_{\mathrm{other}}$ & $Q_{\log}$ & $P_{c,\log}$ [dBm]  \\
    \midrule
        \multirow{2}{*}{AlN\tnote{1}} & run 1 & (3.220 $\pm$ 0.01)$\times 10^{5}$ & -70.2 $\pm$ 0.4  & 0.63 $\pm$ 0.03 & (1.11 $\pm$ 0.01)$\times 10^{5}$ & (2.37 $\pm$ 0.07)$\times 10^{3}$ & -238 $\pm$ 6 \\
        & run 2 & (3.09 $\pm$ 0.01)$\times 10^{5}$ & -68.8 $\pm$ 0.1  & 0.63 $\pm$ 0.01 & (1.13 $\pm$ 0.01)$\times 10^{5}$ & (2.38 $\pm$ 0.02)$\times 10^{3}$ & -238 $\pm$ 2 \\
        \multirow{2}{*}{LiNbO$_{3}$\tnote{2}} & run 1 & (8.42 $\pm$ 0.09)$\times 10^{5}$ & -94.0 $\pm$ 0.2 & 0.59 $\pm$ 0.01 & (1.27 $\pm$ 0.02)$\times 10^{5}$ & 937 $\pm$ 8 & -638 $\pm$ 9  \\
        & run 2 & (8.52 $\pm$ 0.03)$\times 10^{5}$ & -93.8 $\pm$ 0.2 & 0.62 $\pm$ 0.01 & (1.27 $\pm$ 0.01)$\times 10^{5}$ & 969 $\pm$ 9 & -620 $\pm$ 4 \\
    \bottomrule
    \end{tabular*}
    \begin{tablenotes}
        \item [1]{Resonance frequency $\nu_{0}=$ 9.5661021(2) GHz for run 1, $\nu_{0} =$ 9.5546120(3) GHz for run 2.}
        \item [2]{Resonance frequency $\nu_{0}=$ 7.6779852(3) GHz for run 1, $\nu_{0} =$ 7.6752083(4) GHz for run 2.}
    \end{tablenotes}
    
    \label{tab:PwrSweepRegrResultsTM010}
\end{threeparttable}
\end{sidewaystable}

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
